PROVE: Training-Free Prompt Recovery using Verifiable Evidence

Modern text-to-image models can generate highly realistic images from natural-language prompts, while recent advances in prompt inversion have made it increasingly feasible to recover those prompts from generated outputs, raising new concerns for copyright protection and content ownership. As prompt marketplaces emerge, recovered prompts can enable both the unauthorized reproduction and redistribution of copyrighted creative works, and the exposure of the prompts that encode an artist's creative recipe in AI-generated content. Existing prompt inversion methods rely on gradient-based optimization, autoregressive captioning, or reinforcement learning. However, optimization-based methods often produce unreadable prompts, captioning methods hallucinate unverified details, and RL-based approaches frequently overfit to specific generators while introducing evaluation circularity. We introduce PROVE (Prompt Recovery with Verified Evidence), a training-free, black-box prompt inversion attack that reconstructs prompts by composing verifiable scene descriptions rather than optimizing token sequences, targeting both original copyrighted works and AI-generated content. The resulting prompts are fully auditable, with every recovered claim grounded in explicit image evidence, and are formalized through a precision-constrained recall maximization objective. Across MS-COCO, Flickr30K, and Lexica, using state-of-the-art text-to-image generators, PROVE consistently outperforms optimization, captioning, and RL-based baselines on image similarity (DINO, LPIPS) and text-image alignment (CLIP), without any training, generator access, or fine-tuning, demonstrating a stronger and more practical prompt inversion attack.

==> sec/image_prompt_comparison.tex <==
\begin{figure*}[t]
\centering
% ---- Target image, vertically centered against the whole table ----
\begin{minipage}[c]{0.17\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/lexica-art/target.jpg}\\[4pt]
  \textbf{Target}
\end{minipage}\hfill
% ---- Comparison table ----
\begin{minipage}[c]{0.80\textwidth}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.19\linewidth} m{0.75\linewidth}@{}}
\toprule
\textbf{Generated} & \textbf{Recovered prompt} \\
\midrule
\includegraphics[width=\linewidth]{fig/lexica-art/ours_gen.jpg} &
\textbf{Ours.} An open door emits warm light into a dimly lit room with cool blue and orange tones. The walls are plain, and the floor reflects the light, creating a stark contrast between the two halves of the space. Artificial, evening, indoor, eye-level, warm, orange, concrete floor, blurred. It contains three hinges, two walls. Gold handles, open, new, rectangular, smooth. No text, rectangular shape. Hinges. 3D render, minimalist, low-key, muted palette with orange accents, atmospheric, hyperdetailed. \\
\midrule
\includegraphics[width=\linewidth]{fig/lexica-art/pm_gen.jpg} &
\textbf{PromptMiner.} an open door room, darker empty room with open doorway
leading to glowing lit hallway, warm lighting, orange and blue walls, concrete
floor, minimal composition, colorful, minimalist, high-contrast, high resolution. \\
\midrule
\includegraphics[width=\linewidth]{fig/lexica-art/vlm_gen.jpg} &
\textbf{VLM-as-expert.} A minimalist room with two open doors, one glowing warmly
and the other coolly, casting colorful reflections on the concrete floor. \\
\midrule
\includegraphics[width=\linewidth]{fig/lexica-art/cig_gen.jpg} &
\textbf{CLIP-Interrogator.} a door in a room with a light coming in, teal orange
color palette 8k, pexels, high quality fantasy stock photo, low saturated red and
blue light, open door, vanilla-colored lighting, pink and teal and orange. \\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Qualitative comparison on Lexica. We compare \emph{PROVE} against its three closest baselines, showing both the generated image and the recovered prompt. On these stylized images, \emph{PROVE} describes the visual style in grounded terms without attributing it to a named artist, unlike the baselines, which recover artist and platform tags.}
\label{fig:qual_lexica}
\end{figure*}


\begin{figure*}[t]
\centering
% ---- Target image, vertically centered against the whole table ----
\begin{minipage}[c]{0.17\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/ms-coco/target.jpg}\\[4pt]
  \textbf{Target}
\end{minipage}\hfill
% ---- Comparison table ----
\begin{minipage}[c]{0.80\textwidth}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.19\linewidth} m{0.75\linewidth}@{}}
\toprule
\textbf{Generated} & \textbf{Recovered prompt} \\
\midrule
\includegraphics[width=\linewidth]{fig/ms-coco/ours_gen.jpg} &
\textbf{Ours.} A bed with white linens and a metal headboard sits between two windows with closed blinds in a simple bedroom. A nightstand with a lamp and a candle is to the right of the bed. The room has a ceiling fan with lights. Bright, daytime, indoor, eye-level, neutral, plain. It contains three pillows, two fans. Black wrought iron headboard with curved scrollwork. Dark brown wooden nightstand, small glass candle holder, window with white frame, light source from window, shadowed corner, minimalistic. White pillow, soft, slightly wrinkled, on bed, unmade, indoor setting. Wooden frame, window blinds, nightstand lamp. Beige pillow with white pillowcase, slightly wrinkled, soft-looking, on bed with dark metal headboard. Clear glass, smooth surface, transparent, round, empty. Wooden-framed window with horizontal blinds, partially open, allowing natural light into room, white walls visible. \\
\midrule
\includegraphics[width=\linewidth]{fig/ms-coco/pm_gen.jpg} &
\textbf{PromptMiner.} bedroom, cosy bedroom, traditional wooden furniture, twin metal bed, white sheets, soft lighting, window with blinds, hardwood floor, low angle \\
\midrule
\includegraphics[width=\linewidth]{fig/ms-coco/vlm_gen.jpg} &
\textbf{VLM-as-expert.} A cozy bedroom with a metal bed frame, white bedding, wooden blinds, a nightstand with a lamp, and a ceiling fan with lights. \\
\midrule
\includegraphics[width=\linewidth]{fig/ms-coco/cig_gen.jpg} &
\textbf{CLIP-Interrogator.} a bed with a white comforter and a fan in a room, sunlight through windows, photo taken with canon 5d, by Gregory Gillespie, story board format.\\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Qualitative comparison on MS-COCO. We compare \emph{PROVE} against its three closest baselines, showing both the generated image and the recovered
prompt. \emph{PROVE} recovers finer-grained, detailed prompts, which in turn yield reconstructions closer to the target.}
\label{fig:qual_coco}
\end{figure*}

\begin{figure*}[t]
\centering
% ---- Target image, vertically centered against the whole table ----
\begin{minipage}[c]{0.17\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/flickr/target.jpg}\\[4pt]
  \textbf{Target}
\end{minipage}\hfill
% ---- Comparison table ----
\begin{minipage}[c]{0.80\textwidth}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}>{\centering\arraybackslash}m{0.19\linewidth} m{0.75\linewidth}@{}}
\toprule
\textbf{Generated} & \textbf{Recovered prompt} \\
\midrule
\includegraphics[width=\linewidth]{fig/flickr/ours_gen.jpg} &
\textbf{Ours.} A dog stands in shallow water near a sandy shore, its silhouette highlighted by sunlight reflecting off the ripples of the lake. The scene is tranquil, with the dog's reflection visible on the wet sand. Bright, late afternoon, outdoor, eye-level, cool tones, blurred, water reflections. Standing in water, tail up, fur glistening, dark eyes, ears flopped down, legs submerged, water ripples around feet. Wet sand, dark water, ripples, reflections, shoreline. Distorted shapes, unclear details, smooth surface, no text, abstract form, no specific shape, no condition details. \\
\midrule
\includegraphics[width=\linewidth]{fig/flickr/pm_gen.jpg} &
\textbf{PromptMiner.} a grey dog wading in calm water near the shore, reflecting in rippled water; sun reflection, body of calm water; clear day, isometric \\
\midrule
\includegraphics[width=\linewidth]{fig/flickr/vlm_gen.jpg} &
\textbf{VLM-as-expert.} A dog wading in shallow water with sunlight reflecting on the surface, creating sparkling patterns \\
\midrule
\includegraphics[width=\linewidth]{fig/flickr/cig_gen.jpg} &
\textbf{CLIP-Interrogator.} a dog standing in the water, glittering sun rays, ebay photo, by Chippy, 1998 photo, reflections and refractions, backlighted, forced perspective. \\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Qualitative comparison on Flickr30K. We compare \emph{PROVE} against its three closest baselines, showing both the generated image and the recovered prompt. On these natural, caption-style scenes, \emph{PROVE} recovers
finer-grained detailed prompts than the baselines, yielding reconstructions closer to the target.}
\label{fig:qual_flickr}
\end{figure*}





==> sec/qualitative_comparison.tex <==
% \pagestyle{empty}

% % ---- geometry of a single cell -------------------------------------
% \newlength{\cellside}\setlength{\cellside}{2.05cm} % width == height of each thumbnail
% \setlength{\tabcolsep}{1.6pt}                       % horizontal gap between cells
% \newcommand{\rowgap}{1.6pt}                          % vertical gap between image rows
% \newlength{\figwidth}\setlength{\figwidth}{9\cellside+16\tabcolsep+4pt} % total grid width
 
% % highlight colour for the proposed method
% \definecolor{provegreen}{RGB}{0,150,60}
 
% % ---- centre-crop-to-square helper ----------------------------------
% % Scales the image so its SHORTER side equals \cellside, then clips the
% % overflow of the longer side symmetrically -> uniform square, no
% % distortion, works for any aspect ratio without knowing pixel sizes.
% \newlength{\imw}\newlength{\imh}\newlength{\croplen}
% \newcommand{\sq}[1]{%
%   \settowidth{\imw}{\includegraphics{#1}}%
%   \settoheight{\imh}{\includegraphics{#1}}%
%   \ifdim\imw>\imh
%     % landscape: fix height, crop left/right symmetrically
%     \settowidth{\imw}{\includegraphics[height=\cellside]{#1}}%
%     \setlength{\croplen}{(\imw-\cellside)/2}%
%     \ifdim\croplen<0pt\setlength{\croplen}{0pt}\fi
%     \edef\trimspec{\the\croplen\space 0pt \the\croplen\space 0pt}%
%     \expandafter\clipbox\expandafter{\trimspec}{\includegraphics[height=\cellside]{#1}}%
%   \else
%     % portrait / square: fix width, crop top/bottom symmetrically
%     \settoheight{\imh}{\includegraphics[width=\cellside]{#1}}%
%     \setlength{\croplen}{(\imh-\cellside)/2}%
%     \ifdim\croplen<0pt\setlength{\croplen}{0pt}\fi
%     \edef\trimspec{0pt \the\croplen\space 0pt \the\croplen}%
%     \expandafter\clipbox\expandafter{\trimspec}{\includegraphics[width=\cellside]{#1}}%
%   \fi
% }
 
% % ---- one row of 9 method images ------------------------------------
% % #1 = folder path (no trailing slash)   #2 = extension of the Original image
% \newcommand{\gridrow}[2]{%
%   \sq{#1/Original.#2} & \sq{#1/PROVE.png} & \sq{#1/BLIP.png} &
%   \sq{#1/CLIP-IG.png} & \sq{#1/PH2P.png} & \sq{#1/STEPs.png} &
%   \sq{#1/VGD.png} & \sq{#1/VLM-as-Expert.png} & \sq{#1/PromptMiner.png}\\[\rowgap]%
% }
 
% % ---- column-header row ---------------------------------------------
% \newcommand{\colhead}{%
%   \small
%   Original & {\bfseries\color{provegreen}PROVE} & BLIP & CLIP-IG & PH2P &
%   STEPs & VGD & VLM-Expert & PromptMiner\\[2pt]%
% }
 
% % ---- one full dataset block (title + headers + 3 rows) -------------
% % #1 = dataset display name  #2..#4 = the three row folders  #5 = Original ext
% \newcommand{\datasetblock}[6]{%
%   {\rmfamily\bfseries\fontsize{17}{19}\selectfont #1}\par\vspace{3pt}
%   \begin{tabular}{@{}*{9}{c}@{}}
%     \colhead
%     \gridrow{#2}{#6}
%     \gridrow{#3}{#6}
%     \gridrow{#4}{#6}
%   \end{tabular}\par\vspace{16pt}%
% }
 
% % ---- the complete grid, as a single reusable box -------------------
% \newcommand{\qualgrid}{%
%   \begin{minipage}{\figwidth}
 
%     \datasetblock{MS-COCO}%
%       {used_photos_inversion/mscoco/r0_000000131131}%
%       {used_photos_inversion/mscoco/r1_000000066135}%
%       {used_photos_inversion/mscoco/r2_000000099242}%
%       {x}{jpg}
 
%     \datasetblock{Flickr}%
%       {used_photos_inversion/flickr/r0_15010}%
%       {used_photos_inversion/flickr/r1_16246}%
%       {used_photos_inversion/flickr/r2_16529}%
%       {x}{jpg}
 
%     \datasetblock{Lexica}%
%       {used_photos_inversion/lexica/r0_06}%
%       {used_photos_inversion/lexica/r1_024}%
%       {used_photos_inversion/lexica/r2_047}%
%       {x}{png}
 
%   \end{minipage}%
% }


\pagestyle{empty}
% ---- geometry of a single cell -------------------------------------
\newlength{\cellside}\setlength{\cellside}{2.05cm} % width == height of each thumbnail
\setlength{\tabcolsep}{1.6pt}                       % horizontal gap between cells
\newcommand{\rowgap}{1.6pt}                         % vertical gap between image rows
\newlength{\figwidth}\setlength{\figwidth}{9\cellside+16\tabcolsep+4pt} % total grid width

% highlight colour for the proposed method
\definecolor{provegreen}{RGB}{0,150,60}

% ---- centre-crop-to-square helper ----------------------------------
\newlength{\imw}\newlength{\imh}\newlength{\croplen}
\newcommand{\sq}[1]{%
  \settowidth{\imw}{\includegraphics{#1}}%
  \settoheight{\imh}{\includegraphics{#1}}%
  \ifdim\imw>\imh
    \settowidth{\imw}{\includegraphics[height=\cellside]{#1}}%
    \setlength{\croplen}{(\imw-\cellside)/2}%
    \ifdim\croplen<0pt\setlength{\croplen}{0pt}\fi
    \edef\trimspec{\the\croplen\space 0pt \the\croplen\space 0pt}%
    \expandafter\clipbox\expandafter{\trimspec}{\includegraphics[height=\cellside]{#1}}%
  \else
    \settoheight{\imh}{\includegraphics[width=\cellside]{#1}}%
    \setlength{\croplen}{(\imh-\cellside)/2}%
    \ifdim\croplen<0pt\setlength{\croplen}{0pt}\fi
    \edef\trimspec{0pt \the\croplen\space 0pt \the\croplen}%
    \expandafter\clipbox\expandafter{\trimspec}{\includegraphics[width=\cellside]{#1}}%
  \fi
}

% ---- one row of 9 method images ------------------------------------
% #1 = folder path (no trailing slash)   #2 = extension of the Original image
\newcommand{\gridrow}[2]{%
  \sq{#1/Original.#2} & \sq{#1/PROVE.jpg} & \sq{#1/PromptMiner.jpg} &
  \sq{#1/STEPs.jpg} & \sq{#1/VGD.jpg} & \sq{#1/PH2P.jpg} &
  \sq{#1/VLM-as-Expert.jpg} & \sq{#1/BLIP.jpg} & \sq{#1/CLIP-IG.jpg}\\[\rowgap]%
}

% ---- column-header row ---------------------------------------------
\newcommand{\colhead}{%
  \small
  Original & {\bfseries\color{provegreen}PROVE} & PromptMiner & STEPs & VGD &
  PH2P & VLM-Expert & BLIP & CLIP-IG\\[2pt]%
}

% ---- one dataset block (title + headers + 1 row) -------------------
% #1 = dataset display name   #2 = row folder   #3 = Original ext
\newcommand{\datasetblock}[3]{%
  {\rmfamily\bfseries\fontsize{17}{19}\selectfont #1}\par\vspace{3pt}
  \begin{tabular}{@{}*{9}{c}@{}}
    \colhead
    \gridrow{#2}{#3}
  \end{tabular}\par\vspace{16pt}%
}

% ---- the complete grid, as a single reusable box -------------------
\newcommand{\qualgrid}{%
  \begin{minipage}{\figwidth}

    \datasetblock{MS-COCO}%
      {used_photos_inversion/mscoco/r0_000000131131}{jpg}

    \datasetblock{Flickr}%
      {used_photos_inversion/flickr/r2_16529}{jpg}

    \datasetblock{Lexica}%
      {used_photos_inversion/lexica/r0_06}{jpg}

  \end{minipage}%
}
